Deploying SDN in G\'EANT production network

Since the demand for more bandwidth, agile infrastructures and services grows, it becomes challenging for Service Providers like G\'EANT to manage the proprietary underlay, while keeping costs low. In such a scenario, Software Defined Networking (SDN), open hardware and open source software prove to be key components to address those challenges. After one year of development, SDX-L2 and BoD, the SDN-ization of the G\'EANT Open and Bandwidth on Demand (BoD) services, have been brought to the pilot status and G\'EANT is now testing the outcomes on its operational network. In this demonstration, we show BoD and SDX-L2 "going live" at the G\'EANT production infrastructure. The pilots run on the same underlay infrastructure thanks to the virtualization capabilities of the network devices. Provisioning of the services is covered during the demo. In the final steps of the demonstration, we show how the infrastructure is able to automatically manage network events and how it remains operational in the case of fault events.

==> inc/5-ack.tex <==
\section{Acknowledgements}
This work was partly funded by the EU G\'EANT (GN4-2) project \cite{geant} as part of the GÉANT 2020 Framework Partnership Agreement (FPA), the project receives funding from the European Union's Horizon 2020 research and innovation programme under Grant Agreement No. 731122 (GN4-2)

